Towards the Adoption of Anti-spoofing Protocols

Email spoofing is a critical step of phishing, where the attacker impersonates someone the victim knows or trusts. In this paper, we conduct a qualitative study to explore why email spoofing is still possible after years of efforts to develop and deploy anti-spoofing protocols (e.g., SPF, DKIM, DMARC). First, we measure the protocol adoption by scanning 1 million Internet domains. We find the adoption rates are still low, especially for the new DMARC (3.1%). Second, to understand the reasons behind the low-adoption rate, we collect 4293 discussion threads (25.7K messages) from the Internet Engineering Task Force (IETF), a working group formed to develop and promote Internet standards. Our analysis shows key security and usability limitations in the protocol design, which makes it difficult to generate a positive "net effect" for a wide adoption. We validate our results by interviewing email administrators and discuss key implications for future anti-spoofing solutions.

==> Makefile <==
# $Id: Makefile,v 1.7 2014/06/28 01:18:01 Gang Exp $

PACKAGE=IEEEtran

LATEX=latex

BIBTEX=bibtex
BIBFILE=bibliography.bib,astro.bib,wang.bib,anon.bib,social.bib,education.bib,zhao.bib
PAPER=survey

TEXFILES = \
	survey.tex \

PDF = ${TEXFILES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.tex   $(PACKAGE).cls IEEEtranS.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


$(PAPER).pdf: $(PAPER).tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

clean:
	rm -f *.dvi *.aux *.ps *~ *.log *.lot *.lof *.toc *.blg *.bbl *.pdf *.out

